Compressed Sensing Constant Modulus Constrained Projection Matrix Design and High-Resolution DoA Estimation Methods

This paper proposes a compressed sensing-based high-resolution direction-of-arrival estimation method called gradient orthogonal matching pursuit (GOMP). It contains two main steps: a sparse coding approximation step using the well-known OMP method and a sequential iterative refinement step using a newly proposed gradient-descent method. To enhance the recoverability, we further propose an efficient projection matrix design method, which considers the constant modulus constraints imposed by the projection matrix hardware components. Simulation results show the effectiveness of the proposed methods as compared to benchmark algorithms.

==> acronyms.tex <==

  \begin{acronym}
  	\acro{HAD}{hybrid analog-digital}
  	\acro{FD}{fully digital}
  	\acro{SE}{spectral efficiency}
    \acro{WSR}{weighted sum rate}
  	\acro{EE}{energy efficiency }
  	\acro{DBF}{digital beamforming}
  	\acro{ABF}{analog beamforming}
  	\acro{mmWave}{millimeter-wave}
    \acro{IID}{independent and identically distributed}
  	\acro{PS}{phase-shifter}
  	
    \acro{LNA}{low-noise-amplifier}
  	\acro{ADC}{analog-to-digital converter}
  	\acro{DAC}{digital-to-analog converter}
  	\acro{PA}{power-amplifier}
  	\acro{BB}{baseband}
  	
  	
  	\acro{OMP}{orthogonal matching pursuit}
  	\acro{RHS}{right-hand-side}
  	\acro{OCI}{out-of-cell interference}

  	\acro{DBF}{digital beamforming}
  	\acro{HBF}{hybrid beamforming}

  	\acro{LoS}{Line-of-Sight}
    \acro{CS}{compressed sensing}
  	\acro{ULA}{uniform linear array}
  	\acro{BD}{block diagonalization}
  	\acro{AoD}{angle-of-departure}
  	\acro{AoA}{angle-of-arrival}
  	\acro{RF}{radio frequency}

  	\acro{3GPP}{3rd Generation Partnership Project}
  	\acro{CSI}{channel state information}
  	\acro{FDD}{frequency division duplex}
  	\acro{LTE}{long-term evolution}
  	\acro{MIMO}{Multiple-input multiple-output}
  	\acro{MRT}{maximum ratio transmission}
  	\acro{MS}{mobile station}



  	\acro{SINR}{signal-to-interference-plus-noise ratio}

  	\acro{SNR}{signal-to-noise ratio}
  	\acro{SVD}{singular value decomposition}
  	\acro{TDD}{time division duplex}
  	\acro{ZF}{zero-forcing}
  	\acro{EVD}{eigenvalue decomposition}
  	\acro{BS}{base station}
  	\acro{KKT}{karush-kuhn-tucker}
  	\acro{MSE}{mean square error}
  	\acro{MMSE}{minimum mean square error}
  	\acro{WMMSE}{weighted \ac{MMSE}}
  \end{acronym}



